ConSlide: Asynchronous Hierarchical Interaction Transformer with Breakup-Reorganize Rehearsal for Continual Whole Slide Image Analysis

Whole slide image (WSI) analysis has become increasingly important in the medical imaging community, enabling automated and objective diagnosis, prognosis, and therapeutic-response prediction. However, in clinical practice, the ever-evolving environment hamper the utility of WSI analysis models. In this paper, we propose the FIRST continual learning framework for WSI analysis, named ConSlide, to tackle the challenges of enormous image size, utilization of hierarchical structure, and catastrophic forgetting by progressive model updating on multiple sequential datasets. Our framework contains three key components. The Hierarchical Interaction Transformer (HIT) is proposed to model and utilize the hierarchical structural knowledge of WSI. The Breakup-Reorganize (BuRo) rehearsal method is developed for WSI data replay with efficient region storing buffer and WSI reorganizing operation. The asynchronous updating mechanism is devised to encourage the network to learn generic and specific knowledge respectively during the replay stage, based on a nested cross-scale similarity learning (CSSL) module. We evaluated the proposed ConSlide on four public WSI datasets from TCGA projects. It performs best over other state-of-the-art methods with a fair WSI-based continual learning setting and achieves a better trade-off of the overall performance and forgetting on previous task

==> iccv2023/0-abstract_chatgpt.tex <==
%%%%%%%%% ABSTRACT
\begin{abstract}

Whole slide image (WSI) analysis has gained significant attention in the medical imaging community for its potential to enable automated and objective diagnosis, prognosis, and therapeutic-response prediction. 
%
However, in clinical practice, the continuous progress of evolving WSI acquisition technology, the diversity of scanners, and different staining and imaging protocols hamper the utility of WSI analysis models.
%
% However, existing WSI analysis methods usually adopt the static model learning setting, with the insufficient capability of ?adapting to new tasks/datasets over time. 
%
In this paper, we propose the FIRST continual learning framework for WSI analysis, named \textbf{ConSlide} to tackle the challenges of enormous image size, efficient utilization of hierarchical structure, and catastrophic forgetting by progressive model updating on multiple sequential tasks. Our framework contains three key components. First, we design a new Hierarchical Interaction Transformer (HIT) to efficiently model and utilize the hierarchical structural knowledge of WSIs. Second, we develop a novel Breakup-Reorganize (BuRo) rehearsal method specifically for WSI data replay with efficient region storing buffer and WSI reorganizing operation. Finally, we devise a new asynchronous updating mechanism to encourage the patch-level and region-level blocks to learn low-level and high-level knowledge, respectively, during the replay stage, based on a nested cross-scale similarity learning (CSSL) module. We evaluated ConSlide on four public WSI datasets from TCGA projects and demonstrated that our framework outperforms other state-of-the-art methods with a fair WSI-based continual learning setting and achieves a better trade-off of the overall performance and forgetting on previous tasks.


\end{abstract}


==> iccv2023/1-introduction_chatgpt.tex <==
\section{Introduction}

Whole slide images (WSIs) contain rich histopathological information of the tissue sections and are routinely used for clinical practice.
% 
With recent advances in deep learning, computational WSIs have garnered significant attention in the medical image analysis community for their potential to provide automated and objective diagnosis, prognosis, and therapeutic-response prediction~\cite{cornish2012whole,lu2021data,shao2021transmil,tanizaki2016report}. 
%
However, the huge size and expensive pixel-level annotations required for WSI analysis present significant computational challenges in architecture design~\cite{lu2020capturing,huang2022deep,javed2020multiplex}.
%Moreover, WSI datasets usually only have slide-level labels, as manual pixel-level annotations of WSI need more effort to obtain, like time, expense, and specific knowledge of pathologist~\cite{liu2017detecting,guan2022node}.
%
To address this issue, multiple instance learning (MIL)-based approaches have been proposed for weakly-supervised WSI analysis~\cite{campanella2019clinical,lu2021data,shmatko2022artificial}, where they first divide WSI into a group of patches, conduct analysis for each patch, and then aggregate them together for slide-level prediction.


\begin{figure}[t]
\centering
\includegraphics[width=0.45\textwidth]{iccv2023/figures/intro_fig.pdf} 
\caption{Illustration of concept and challenges of continual WSI analysis. (a) Continual WSI learning aims to alleviate \textit{catastrophic forgetting} while exploiting knowledge from \textit{sequentially incoming} tasks/datasets. (b) The hierarchical structure of WSIs raises challenges for network architecture and learning strategy design.}
\label{fig:intro}
\vspace{-0.4cm}
\end{figure}


Although encouraging results are achieved, these approaches typically adopt the \textit{static model learning} setting~\cite{li2021dual,shao2021transmil,zhang2022dtfd,chen2022scaling,zheng2022kernel,guan2022node}. However, WSI imaging technology and staining and imaging protocols are subject to an ever-evolving environment, requiring WSI analysis methods to adapt to remain effective~\cite{perkonigg2021dynamic,lee2020clinical}.
%with the insufficient capability of adapting their behaviors to new tasks/datasets over time, and thus require re-training when facing new WSI tasks or datasets~\cite{de2021continual}. 
Unfortunately, preserving previous datasets for continual learning is difficult and impractical due to privacy and storage limitations. A naive solution is to fine-tune a pre-trained model on newly arrived datasets.
%However, there are large discrepancies in the imaging protocols and the equipment across different sites~\cite{mahdi2022lifelonger}, and there are also large differences in morphological characteristics of cells or tissues of different tumors. Thus, the sequentially arrived datasets are normally heterogeneous with considerable domain shifts.
However, during fine-tuning, the network can become too focused on adapting to the feature domain of the current dataset, leading to disruptions in the knowledge acquired from previous tasks/datasets and poor performance on those tasks. 
%
This phenomenon is known as \textit{catastrophic forgetting}~\cite{boschini2022transfer,de2021continual,lesort2020continual}.

%With the increasingly common deployment of WSIs analysis models in both research and clinical settings, 
% Although previous deep learning approaches can get impressive results in tumor sub-typing or survival prediction tasks, they are obtained with static models incapable of adapting their behavior over time, 
%
% However, gathering large enough WSIs datasets is difficult due to discrepancies in the imaging protocols and the equipment across different site~\cite{mahdi2022lifelonger}.
%
% \ylq{Therefore, a naive solution/common solution is to fine-tune the model trained on one tasks/datasets to another tasks/datas}
% \ylq{Add one sentence like above}
%
% However, in practical application, the former\ylq{former? change another word?} WSIs may become intractable due to privacy issues, or may only be available with a few WSIs due to the limitation of storage space. 
%
% In these cases, the model may suffer from catastrophic forgetting of old concepts as new ones are learned, since the models fit the current input data distribution to the the detriment of previously acquired knowledge~\cite{boschini2022transfer,de2021continual,lesort2020continual}.
% \ylq{Maybe you can refer to https://ieeexplore.ieee.org/document/9908146 to organize the logic of this paragraph.}


\textit{Continual Learning} (CL) has been proposed~\cite{lopez2017gradient,de2021continual} as a solution to the limitations of static model learning and catastrophic forgetting.
%
The aim of CL is to train models with adaptability when meeting new tasks without forgetting the knowledge learned from previous tasks catastrophically, which can make deep learning models much more versatile to the constant growth of medical datasets.
%
%CL is widely researched in the field of natural images, either by using parameter regularization~\cite{kirkpatrick2017overcoming,rebuffi2017icarl,kurle2019continual}, knowledge distillation~\cite{li2017learning,fini2022self,boschini2022class}, and appositely designed architectures~\cite{loo2020generalized,pham2021dualnet,douillard2022dytox}, or by storing and replaying previously saved data~\cite{prabhu2020gdumb,buzzega2020dark,cha2021co2l}. 
%
CL has received significant attention in recent years, and it can be achieved through various methods, such as parameter regularization~\cite{kirkpatrick2017overcoming,rebuffi2017icarl,kurle2019continual}, knowledge distillation~\cite{li2017learning,fini2022self,boschini2022class}, apposite architecture design~\cite{loo2020generalized,pham2021dualnet,douillard2022dytox}, or by data rehearsal-based strategies~\cite{prabhu2020gdumb,buzzega2020dark,cha2021co2l}.
%
Among these strategies, rehearsal-based methods have achieved good performance by replaying a subset of the training data stored in a memory buffer.
% \ylq{something like this}
%
However, the characteristics of WSI pose unique challenges for designing continual WSI analysis frameworks and we are not aware of such frameworks in the literature.


WSIs are commonly stored at various resolutions, resulting in a hierarchical structure with containing different pathological information, as depicted in Figure~\ref{fig:intro} (b). 
%
% Images at different resolutions usually contain different histological information. 
%
For example, patch-level images encompass find-grained cells and tumor cellularity information~\cite{GrahamVRATKR19,Pati2020HACTNetAH,DBLP:conf/iccv/AbousamraBAAYGK21}, region-level images mainly characterize the tissue information, such as the extent of tumor-immune localization~\cite{abduljabbar2020geospatial,chen2022scaling,brancati2022bracs}, 
%in representing tumor-infiltrating versus tumor-distal lymphocytes
while slide-level images depict the overall intra-tumoral features~\cite{balkwill2012tumor,javed2020cellular,marusyk2012intra}. 
%Recent works also show that hierarchical models can achieve performance improvement in WSI analysis by utilizing its hierarchical characteristic, and organzing these features in an efficient way~\cite{hou2022h2,chen2022scaling,PatiJFFASBFDRBP22}. 
WSI analysis necessitates modeling and utilizing this hierarchical characteristic~\cite{hou2022h2,PatiJFFASBFDRBP22}, but it is challenging to design a continual WSI analysis framework that can handle this structure.
Our preliminary experiments revealed that directly adapting current CL approaches to hierarchical WSI models results in significant knowledge forgetting of previous tasks (see Section~\ref{Comparison Results}).
%
Moreover, WSIs are gigapixel images with only slide-level labels, which presents storage and computational challenges for rehearsal-based CL, as it is impractical to store and replay the representative WSI in the limited memory buffer.
%and the weak slide-level labels further hinders us to store the representative region information of WSIs.

\if 0
In one hand, WSIs are gigapixel images~\cite{lu2020capturing,huang2022deep,javed2020multiplex} with fine-grained information, which brings computational challenges in model design. The traditional CNN or ViT~\cite{dosovitskiy2020image} architectures cannot be directly applied due to memory limitation. 
%
Second, WSI datasets usually only have slide-level labels. Pixel-level annotations are usually missing,
since manual annotations require non-trivial effort and specific knowledge of pathology~\cite{liu2017detecting,guan2022node}.
%
% Therefore, the common way for WSIs analysis is to split each WSI into a group of patches, and further utilize multiple-instance learning (MIL) model to aggregate patch level features and learn effective representations~\cite{campanella2019clinical,lu2021data,shmatko2022artificial}.\ylq{after reading this sentence, it seems that it is not a challenge... as we alrady have MIL to solve it...}
%
Third, WSIs are usually stored at different resolutions, resulting a hierarchical structure as shown in Figure~\ref{fig:intro} (a). Images at different resolutions usually contain different histological information. 
%
For example, patch-level images encompass information about find-grained features such as cells and tumor cellularity~\cite{GrahamVRATKR19,Pati2020HACTNetAH,DBLP:conf/iccv/AbousamraBAAYGK21}. 
Region-level images mainly characterize information of tissues, such as the extent of tumor-immune localization in representing tumor-infiltrating versus tumor-distal lymphocytes~\cite{abduljabbar2020geospatial,chen2022scaling,brancati2022bracs}. And the slide-level images can depict the overall aggregated features of region-level tissues~\cite{balkwill2012tumor,javed2020cellular,marusyk2012intra}. 
%
Recent works also show that hierarchical models can achieve performance improvement in WSI analysis by utilizing its hierarchical characteristic, and organzing these features in an efficient way~\cite{hou2022h2,chen2022scaling,PatiJFFASBFDRBP22}. 
However, it is non-trivial to utilize the hierarchical structure to benefit the CL problem in WSI analysis. 
Our experiments revealed that directly apply current hierarchical models to CL setting will lead to dramatical knowledge forget about previous tasks.
%%
% Recent research such as H$^2$-MIL~\cite{hou2022h2} propose to regard the WSI pyramid structure as a heterogeneous graph with the "resolution" attribute to explicitly model the features and spatial-scaling relationships of multi-resolution patches. Since the heterogeneous graph is constructed by the spatial relation between patches, it usually lacks the insights in analyzing global information interactions. HIPT~\cite{chen2022scaling} is another promising framework for the analysis of WSIs, which leverages the natural hierarchical structure inherent in WSIs using three levels of Transformer structure~\cite{vaswani2017attention}. Nevertheless, the HIPT largely relies on pre-training and it neglect the coarse-grained features that obtained from region-level images directly.
\fi 


%
%To tackle these limitations, in this paper, we present a novel domain-incremental learning framework to enable progressive updates of cardiac image segmentation model with effective exploration of the sequentially arrived heterogenous data from multiple sites. In each time step, the updated model does not catastrophically forget past domains and can well adapt to current domains and unseen domains.
To tackle these challenges, we develop a novel WSI continual analysis framework, named \textit{ConSlide} to enable progressive update of a hierarchical WSI analysis architecture by sequentially utilizing the heterogeneous WSI datasets from multiple tasks.
%store representative regions during the training process of current task, and replay the augmented WSIs which are reorganized by the saved regions. In this way, the knowledge learned from previous tasks can be preserved, while the model being updated through an asynchronous mechanism.
%
We achieve this by storing a representative region set of past tasks, and then regularly reorganizing and replaying them during the current model update with an asynchronous updating mechanism.
%
Specifically, we first design a novel \textit{Hierarchical Interaction Transformer} (HIT) as the backbone to model and utilize the hierarchical characteristic of WSIs efficiently. 
%
HIT aggregates both fine-grained and coarse-grained WSI features to enable more comprehensive WSI analysis via its bidirectional interaction within the hierarchical structure. 
%
Further, to facilitate the continual update of the designed hierarchical architecture, we follow the rehearsal strategy and develop a novel \textit{Breakup-Reorganize} (BuRo) rehearsal module that addresses the unique challenges of WSI data replay.
%
Particularly, the BuRo rehearsal module utilizes the random sampling strategy to select and store WSI regions of old tasks efficiently, and then reorganize augmented WSIs of old tasks to improve the knowledge fidelity of old tasks in the replay step.
%
Based on the augmented old task WSI data, we further devise a new asynchronous updating mechanism to encourage the patch-level and region-level blocks to learn more task-agnostic and task-specific knowledge, respectively, by conducting a nested \textit{Cross-Scale Similarity Learning} (CSSL) task from both old and current WSI data.

With the above careful designs, our framework can preserve the knowledge of previous WSI tasks to mitigate catastrophic forgetting and improve the generalization of the WSI model for more accurate analysis. 
%%
We evaluated our framework on four public WSI datasets from TCGA projects and conducted extensive ablation analysis to demonstrate the effectiveness of each proposed module. 
Importantly, our \textit{Conslide} outperforms other comparison methods and achieves a better trade-off of the overall performance and forgetting on previous tasks under a fair WSI CL setting. Our code is available at \href{https://anonymous.4open.science/r/ConSlide}{https://anonymous.4open.science/r/ConSlide}.

==> iccv2023/2-relatedwork_chatgpt.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.9\textwidth]{iccv2023/figures/model_structure.pdf} 
% Reduce the figure size so that it is slightly narrower than the column. Don't use precise values for figure width.This setup will avoid overfull boxes.
\caption{Illustration of our proposed continual WSI analysis framework. (a) The architecture and whole process of our proposed \textit{ConSlide} framework, which includes \textit{Training}, \textit{Storing}, and \textit{Replay}. (b) The details of our proposed Breakup-Reorganize (BuRo) rehearsal method. (c) Illustration of the proposed Cross-Scale Similarity Learning (CSSL) module.}
\label{fig:model}
\vspace{-0.3cm}
\end{figure*}

\section{Related Work}

\para{Multiple Instance Learning for WSI Analysis.}
Multiple Instance Learning (MIL) has been widely adopted for WSI analysis.
In the conventional MIL approach, handcrafted aggregators such as mean-pooling or max-pooling are used to obtain bag-level representations. 
%Due to the sensitivity to singular values, these handcrafted aggregators are easily to be affected by some strange features. 
Recently, attention-based aggregators have shown great potential.
%
For example, Ilse \textit{et al.}~\cite{ilse2018attention} proposed an attention-based MIL model that obtains the bag embedding by considering the contribution of each instance.
Campanella \textit{et al.}~\cite{campanella2019clinical} further extended this strategy to WSI analysis. 
%
Lu \textit{et al.}~\cite{lu2021data} developed an attention-based global pooling operator for weakly-supervised WSI classification by using ResNet-50 as the instance-level feature extraction. 
%
%However, the performance of attention-based aggregators may be affected by some instances that are irrelevant to the classification task. 
Moreover, Li \textit{et al.}~\cite{li2021dual} extended the attention-based aggregators for WSI analysis by combining the max pooling operator and attention-based aggregators with a simple summation.
%, and proved that the handcrafted aggregators are also important for MIL in WSIs analysis.

\para{Hierarchical Structure in WSI.}
To leverage the pyramid structure information of WSIs, Li \textit{et al.}~\cite{li2021dual} proposed a multi-scale MIL model that extracts patches at two different resolutions and concatenates features from different resolutions in a pyramidal way. 
%
Hou \textit{et al.}~\cite{hou2022h2} proposed a hierarchical graph neural network to model the pyramid structure of WSIs. 
%
Recently, Chen \textit{et al.}~\cite{chen2022scaling} proposed a hierarchical Transformer (\ie, HIPT) to leverage the natural hierarchical structure in WSIs. 
%
However, HIPT only uses fine-grained features to obtain coarse-grained features and lacks interaction between the two levels.
% \ylq{However, the different level features in HIPT are trained separately and there is no interaction}. Done
%
In contrast, our proposed HIT model implements a novel bidirectional information interaction between patch- and region-level features, allowing for a more effective and accurate WSI analysis.
%Although achieving promising performance, Transformer-based models usually suffer from low computation efficiency, and the needs for pre-training and parameter freezing may significantly limit their deployment in end-to-end training scenarios. 
%%%%%%
% Recent research such as H$^2$-MIL~\cite{hou2022h2} propose to regard the WSI pyramid structure as a heterogeneous graph with the "resolution" attribute to explicitly model the features and spatial-scaling relationships of multi-resolution patches. Since the heterogeneous graph is constructed by the spatial relation between patches, it usually lacks the insights in analyzing global information interactions. HIPT~\cite{chen2022scaling} is another promising framework for the analysis of WSIs, which leverages the natural hierarchical structure inherent in WSIs using three levels of Transformer structure~\cite{vaswani2017attention}. Nevertheless, the HIPT largely relies on pre-training and it neglect the coarse-grained features that obtained from region-level images directly.

\para{Continual Learning for Medical Image Analysis.}
Continual learning has gained significant attention in the machine learning and computer vision community recently.
%
Various scenarios of continual learning exist, such as class-incremental learning, task-incremental learning, and domain-incremental learning.
%
The continual learning strategies can be divided into several categories: regularization-based~\cite{aljundi2018memory,kirkpatrick2017overcoming,li2017learning,zenke2017continual,rebuffi2017icarl,kurle2019continual}, distillation-based~\cite{li2017learning,buzzega2020dark,fini2022self,boschini2022class}, 
architecture design-based~\cite{li2019learn,loo2020generalized,wortsman2020supermasks,pham2021dualnet,douillard2022dytox}, 
and rehearsal-based~\cite{chaudhry2019tiny,prabhu2020gdumb,wu2019large,buzzega2020dark,cha2021co2l}. 
%
For a comprehensive review of continual learning, interested readers can refer to~\cite{de2021continual}
%
Recently, there have been some works studying the CL setting in medical image analysis, such as CL for MRI detection and classification~\cite{baweja2018towards,perkonigg2021dynamic,ozgun2020importance}, X-ray classification on chest~\cite{lenga2020continual}. 
%
Particularly, some recent works discuss the benchmark of CL in pathology~\cite{mahdi2022lifelonger,kaustaban2022characterizing}. 
However, these works are limited in patch-level WSI analysis due to obstacles brought by the gigapixel nature of WSIs.
%
As far as we know, this research is the first one to discuss the challenges and solutions of continual slide-level pathology analysis.

==> iccv2023/3-methods_chatgpt.tex <==
\section{Problem Formulation}

\para{WSI Preprocessing.}
WSIs can be formed in a hierarchical structure, \eg, WSI-, region-, and patch-level, respectively.
%
For an original WSI $\mathcal{I}$, we split it into $M$ non-overlapping regions $\mathcal{R}$ with size of $4,096\times 4,096$, and each region is further split into $N$ non-overlapping patches $\mathcal{P}$ with size of $512\times 512$, where $\mathcal{I} = [\mathcal{R}_{1}, \mathcal{R}_{2},  \cdots, \mathcal{R}_{M}]$, and $\mathcal{R}_{i} = [\mathcal{P}_{i1}, \mathcal{P}_{i2},  \cdots, \mathcal{P}_{iN}], 1 \leq i \leq M$. 
The regions $\mathcal{R}$ are stored in a downsampling version in which we re-scale the size from $4,096 \times 4,096$ to $512 \times 512$ for downstream processing.
%
To ease the training, we extract the \textit{patch-level} features $\boldsymbol{P}$ from $\mathcal{P}$ and the \textit{region-level} features $\boldsymbol{R}$ from $\mathcal{R}$ with a pre-trained feature extractor, \eg, ConvNeXt~\cite{liu2022convnet}.
%
Therefore, we can obtain the region-level and patch-level features with the following format $\boldsymbol{R} = [\boldsymbol{R}_1, \boldsymbol{R}_2,  \cdots, \boldsymbol{R}_M]$, $\boldsymbol{P}_{i} = [\boldsymbol{P}_{i1}, \boldsymbol{P}_{i2},  \cdots, \boldsymbol{P}_{iN}]$, and $ \boldsymbol{P}_{ij}, \boldsymbol{R}_{i} \in \mathbb{R}^{1 \times C}$, where $C$ means feature channels.


\para{Continual Learning for WSI Analysis.}
CL for WSIs is defined as training a model on non-stationary WSI datasets with a series of tasks/classes/domains.
%
We define a sequence of datasets $\mathcal{D}=\left\{\mathcal{D}_1, \mathcal{D}_2, \cdots, \mathcal{D}_T\right\}$, where the $t$-th dataset $\mathcal{D}_t=\{\boldsymbol{x}, y, t\}_k$ contains tuples of the WSI sample $\boldsymbol{x}$, its corresponding label $y$, and optional datasets identifier $t$. In the class-incremental scenario, the model needs to predict the classification label $y$ with WSI $\boldsymbol{x}$ as the input, while in the task-incremental scenario, the inputs are the combination of WSI $\boldsymbol{x}$ and its corresponding task identifier $t$.


\section{Method}

Our rehearsal-based continual WSI analysis framework is shown in Figure~\ref{fig:model} (a), which includes three steps: \textbf{Training}, \textbf{Storing}, and \textbf{Replay}. 
%
1) We train the proposed \textit{Hierarchical Interaction-based Transformer (HIT)} model with the current dataset (and replay data) in the \textbf{Training} step.
%
2) We adopt the proposed \textit{Breakup-Reorganize (BuRo)} scheme to store a representative set of WSI regions from current datasets to buffer in the \textbf{Storing} step.
3) We \textbf{Replay} the stored WSI data and employ the proposed \textit{asynchronous updating} paradigm to remind the model of the previous dataset knowledge in the next training step.
The whole pipeline is conducted in a closed-loop manner.

\subsection{Hierarchical Interaction Transformer (HIT)}
Different from natural images, WSIs are gigapixel images with a hierarchical structure.
%
Therefore, we design a powerful Hierarchical Interaction-based Transformer model to abstract the hierarchical structural information of WSI.
%
As shown in Figure~\ref{fig:model} (a), the proposed HIT model consists of $L$ layers, where each layer contains three components: Patch-level Transformer (PT) block, Region-level Transformer (RT) block, and Hierarchical Interaction (HI) block.
%
The PT and RT blocks are used to aggregate the patch-level and region-level features, while the HI block is employed to conduct the interaction between these two level blocks.
%

\para{Patch-level Transformer Block.}
Given the patch-level feature set $\boldsymbol{P}^{l-1}_i$ of the $i$-th region $\mathcal{R}_{i}$, the PT block learns the relationship of different patch features in this region and then calculates the output feature
\begin{equation}
\hat{\boldsymbol{P}}^{l}_i = {\rm PT}\left(\boldsymbol{P}^{l-1}_i\right),
\end{equation}
where $l = 1, 2, ..., L$ is the index of the HIT block.
%
${\rm PT}(\cdot)$ is one layer canonical Transformer~\cite{dosovitskiy2020image}, including Multi-head Self-Attention (MSA), Multi-Layer Perceptron (MLP), and Layer Normalization (LN).
%
The PT blocks share the same parameters among all patches in the same layer. 

\para{Hierarchical Interaction Block.}
We further design a HI block to fuse the patch-level features and region-level features of the same region in a bidirectional manner. 
%
Specifically, for region $\mathcal{R}_{i}$ in the $l$-th HIT block, we have its region-level feature $\boldsymbol{R}^{l-1}_i$ and the output feature of the PT block $\hat{\boldsymbol{P}}^{l}_i$ in this layer. 
%
To get the interacted patch-level feature $\boldsymbol{P}^{l}_i$, we add $\boldsymbol{R}^{l-1}_i$ to $\hat{\boldsymbol{P}}^{l}_i$.
%
To get the interacted region-level feature $\hat{\boldsymbol{R}}^{l}_i$, we first process the patch-level features $\hat{\boldsymbol{P}}^{l}_i$ with a convolution and a max pooling operator and then add the processed patch-level feature to the region-level feature $\boldsymbol{R}^{l-1}_i$.
%
The procedure can be represented as
\begin{equation}
\begin{split}
    \boldsymbol{P}^{l}_i &= \hat{\boldsymbol{P}}^{l}_i + \boldsymbol{R}^{l-1}_i, \\
    \hat{\boldsymbol{R}}^{l}_i &= \boldsymbol{R}^{l-1}_i + {\rm Max}\left({\rm Conv}\left(\hat{\boldsymbol{P}}^{l}_i\right)\right).
\end{split}
\end{equation}
%
Similar to the PT block, the HI blocks also share the same parameters among all patches in the same layer. 

\para{Region-level Transformer Block.}
The final process in our HIT model is to learn the relationship of the interacted region-level features generated from HI blocks. 
%
Specifically, the RT block handles the interacted region-level feature set of $M$ regions $\hat{\boldsymbol{R}}^{l} = [\hat{\boldsymbol{R}}^{l}_1, \hat{\boldsymbol{R}}^{l}_2, \cdots, \hat{\boldsymbol{R}}^{l}_M]$, and calculates the output feature 
\begin{equation}
    \boldsymbol{R}^{l}_i = {\rm RT}\left(\hat{\boldsymbol{R}}^{l}_i\right).
\end{equation}
%
Similar to the PT block, ${\rm RT}(\cdot)$ is also one layer canonical Transformer. 
We take the first token of the RT block output at the last layer as the slide-level representation, and then use a linear layer to generate the final slide-level prediction.


%
\noindent\faIcon{bullhorn} \textbf{Discussion.}
Our proposed HIT model is different from previous hierarchical transformer~\cite{chen2022scaling}. 
We design a novel bidirectional information interaction block between the patch- and region-level features so that our network can model WSI in a more effective and accurate manner.

\subsection{Breakup-Reorganize Rehearsal Method}

Existing rehearsal-based CL methods usually save the whole natural images to the buffer, which is not suitable for gigapixel WSIs.
%
As WSI can be split into non-overlapping regions, we propose a novel rehearsal method, named \textit{Breakup-Reorganize} (RuRo), as shown in Figure~\ref{fig:model} (b) and Algorithm~\ref{alg1}. 

\para{Breakup.} For each WSI, we first sample some regions randomly, and store these regions in the buffer.
%
We highlight that, instead of the original image, the buffer stores region-level features $\boldsymbol{R}_i$ and their corresponding patch-level features $\boldsymbol{P}_i$.

\para{Reorganize.}
During the replaying step, according to a given pair of task id and label each time, we will randomly sample $n$ regions which have the same task id and label from the buffer. 
Then we reorganize the selected regions to form a new augmented WSI.

\noindent\faIcon{bullhorn} \textbf{Discussion.} We argue that our proposed BuRo method has three advantages.
1) BuRo is resource efficient in continual WSI analysis scenarios, especially when buffer size is limited, as it can store regions from a bigger number of WSI sources;
2) BuRo can boost the diversity of the buffered data by preserving diverse knowledge from previous tasks;
and 3) \textit{Reorganize} operation promotes the generalization ability of the model, as it generates new WSIs with a large number of potential combinations, which means that BuRO is able to ``increase" the sample size without any extra buffer size.


\begin{algorithm}[!t]
	%\textsl{}\setstretch{1.8}
	\renewcommand{\algorithmicrequire}{\textbf{Initialize:}}
	\renewcommand{\algorithmicensure}{\textbf{Output:}}
	\caption{The process of proposed BuRo Method}
	\label{alg1}
	\begin{algorithmic}[1]
	    \REQUIRE dataset $\mathcal{D}$, model $f$, loss function $\ell$, scalar $\alpha$
		\STATE $\mathcal{M} \gets \{\}$
		\FOR {$\mathcal{D}_t$ in $\mathcal{D}$}
            \FOR {$(x_k, t_k, y_k)$ in $\mathcal{D}_t$}
                \STATE  $(\mathcal{R}^{'}, t^{'}, y^{'}) \gets Select(\mathcal{M})$
                \STATE $x^{'} \gets Reorganize(\mathcal{R}^{'})$
                \STATE $loss = \ell(y_k, f(x_k)) + \alpha\ell(y^{'}, x^{'})$
                \STATE $\mathcal{R}^{''} = Sample(Breakup(x_k))$
                \STATE $\mathcal{M} \gets Reservoir(\mathcal{R}^{''}, t_k, y_k)$
            \ENDFOR
        \ENDFOR
% 		\ENSURE  decomposed modes $ \left\{ {{s_k}\left( t \right)} \right\}$, $\left\{ {{\omega _k}\left( t \right)} \right\}$
	\end{algorithmic} 
\end{algorithm}
% \vspace{-0.3cm}
% \subsection{Cross-Scale Similarity Learning for Asynchronous Updating}
\subsection{Asynchronous Updating with Cross-Scale Similarity Learning}

\if 0
Although HIT model performs better than other start-of-the-art models, it may suffer from catastrophic forgetting in CL. However, during our experiments, we find it can mitigate the catastrophic forgetting of HIT model by just using the region-level features and RT block for training. 
%
Besides, the HIPT~\cite{chen2022scaling} model, which has three-tier hierarchical structure, can get good performance by training the network level-by-level, since it's hard to converge by end-to-end training. From these, we can draw the hypothesis that the hierarchical structure may reduce the robustness of HIT model in CL scenario. 
%

Furthermore, we are inspired by the classic \textit{Complementary Learning System (CLS)} theory~\cite{kumaran2016learning,mcclelland1995there}.
The theory suggests that humans continually learn via cooperation of two learning systems, the "hippocampus" and "neocortex". 
Hippocampus focuses on learning pattern-separated representation of specific task, and we denote it as \textit{Special-learner}. 
Neocortex focuses on learning more basic and general representation from previous experience, and we name it as \textit{General-learner}. 
With these two systems, CLS can adapt to new task while preserving most general knowledge of old tasks, mitigating catastrophic forgetting.
%
There are several CL methods designed on the basis of CLS~\cite{pham2021dualnet,wang2022dualprompt}.
%
\begin{comment}
Inspired by the theory, we noticed that our proposed HIT model can also be regarded as a CLS: PT block can be regarded as General-learner learning general knowledge in patch-level, while RT block can be treated as Special-learner learning task specific knowledge in region level.
\end{comment}
%
However, the RT block faces a more challenging situation. 
%
On one hand, the RT block needs to adapt its way of feature aggregation to the new task.
On other other hand, the RT block also needs to adapt to the updates of the PT block mentioned above.
%
Therefore, there is great possibility that the RT block will forget a vast knowledge of previous task when the new task arrives. 
%
Although non-hierarchical model can mitigate forgetting, however, it is unable to capture fine-grained features of WSI in region-level. 

To address this problem, we first randomly initialize and freeze the parameters of PT block of HIT model. 
%
Surprisingly, the HIT model can alleviate the catastrophic forgetting while keep most of ability to capture WSI features.

How to train the PT block as a General-learner? 
The most intuitive way is to train PT block with Self-Supervised Learning~(SSL) tasks. 
However, most current SSL methods are designed for natural images, they learn embeddings which are invariant to distortions~\cite{zbontar2021barlow,bardes2021vicreg}, and are not suitable for WSIs which are gigapixel and have hierarchical structure. 
%
Although HIPT~\cite{chen2022scaling} proposed to pre-train the model with WSIs in self-supervised manner by using DINO~\cite{caron2021emerging}, which encourage local-to-global correspondences between student and teacher, it may causes the model to learn similar patch-level and region-level features, and thus discards learning more fine-grained features. 
%
Besides, it is hard to integrate the continual learning process organically. 
\fi 


In our proposed HIT architecture, the PT blocks are mainly used to extract low-level morphology features, while the RT blocks are mainly used to extract high-level task-specific semantic features.
%
During the ideal continual learning process, the PT blocks should be updated \textit{slowly} since most tasks share low-level morphology features, while RT blocks need to be learned \textit{quickly} on the new task to extract the task-specific discriminative features.
%
To enable that, we design a new Cross-Scale Similarity Learning (CSSL) scheme and assign smaller loss weight for PT block to encourage \textit{asynchronous updating} of the PT block and RT block parameters.


Formally, given a WSI image, we use a linear projector to project its region-level features into region-level projections, and then calculate the cosine similarity among the $M$ region-level projections to form a similarity matrix $\mathcal{C}^r \in \mathbb{R}^{M\times M}$.
%
Meanwhile, for the patch-level features of the same WSI image, we take the average of the PT block output features within the same region as the ``second" region-level features.
We then use the same linear projector to project them into projections and calculate the second cosine similarity matrix $\mathcal{C}^p \in \mathbb{R}^{M\times M}$ with acquired ``second" region-level projections. 
%
The objective of the CSSL is to minimize the Mean Squared Error (MSE) loss between these two similarity matrices from different levels:
\begin{equation}
\mathcal{L}_{CSSL}=\sum_{i}\sum_{j}(\mathcal{C}^r_{ij}-\mathcal{C}^p_{ij})^2.
\end{equation}

During the training phase, we conduct the proposed CSSL on the replayed and current WSI data and utilize this supervision to update the PT block parameters.
%
Also, we calculate the final slide-level prediction loss on the current WSI data and utilize this supervision to update the network parameters.
%
In this case, the PT blocks need to simultaneously perform well on replayed data and current data, so that they are encouraged to retain the common low-level knowledge.
Meanwhile, the RT blocks need to perform well on the current dataset, so that they are encouraged to adapt their parameters to the new task.

\noindent\faIcon{bullhorn} \textbf{Discussion.} We note that the CSSL module constrains the consistency between region- and patch-level matrices calculated by region- and patch-level features respectively, which will not constrains the consistency between region- and patch-level features themselves. Although our asynchronous updating paradigm is inspired by the classic complementary learning system~\cite{buzzega2020dark, pham2021dualnet}, we specifically take advantage of the natural hierarchical structure to design our asynchronous updating paradigm, which avoids explicitly adopting two steps/models and further improves the learning efficiency.

